Quick-View Takeaways: How Does Title Framing Influences Pattern Identification in Line Charts?

Visual data communication in digital media is increasingly characterized by short attention spans and snapshot-based viewing, often employing line charts to convey trends and patterns. Among all visual elements, titles are crucial ones that can shape how viewers interpret visual information and form chart takeaways. In this study, we examine how title characteristics, particularly title word count and intended message, influence people's pattern identification in single-class line charts. Participants viewed 50 line charts collected from online news media and identified the pattern they perceived. Our results demonstrate that both title word count and intended message significantly influence viewers' pattern identification. Our findings highlight the importance of title design in shaping chart takeaways and effective visualization communication.

==> sections/2-related.tex <==
% \subsection{Analytical Task on Line Graphs}

% Add here previous perceptual and empirical studies with low-level task~\cite{amar2005lowLevelComponentsInfoVis} on line graphs.

% Take some reference from the LineSmooth and the Visual Steganography paper.
\noindent \textbf{Visual Pattern Perception in Line Charts}
How viewers perceive and describe patterns in time-series graphics is a cornerstone problem of graphical perception initiated by Cleveland and McGill~\cite{cleveland1988shape}.
Foundational work demonstrates that people heavily rely on geometric properties, especially slopes and changes, to identify information in line charts~\cite{talbot2012empirical, wang2017there, moritz2023average}.
People naturally employ natural-language descriptors for such slopes and changes, using terms like “soaring” and “tanking,” and these descriptors can be systematically mapped to underlying geometric properties of line charts~\cite{bromley2023differencemountainmolehillquantifying}.
Building on this understanding, researchers have operationalized this semantic language for interaction, enabling users to search for trends in datasets using qualitative terms such as "sharp increase" or "gradual decline"~\cite{bendeck2024slopeseeker}.
% 
Users' perceptual thresholds play a critical role in visual perception~\cite{wang2025characterizing, szafir2017modeling}.
Detecting subtle differences in slopes can be harder when too many lines appear in a single chart~\cite{moritz2018visualizing} or are placed together by other textual factors such as captions~\cite{kim2021understandingReadersIntegrateChartsCaptions}. In this work, we examine how different dimensions of title design features affect rapid judgment. 
% The visual complexity of a line chart further influences rapid judgment and accuracy. Evidence suggests that cluttered or noisy patterns reduce perceptual performance under time constraints, leading viewers to rely on heuristic interpretations rather than precise visual analysis~\cite{ryan2018glancepixelapproximateentropy, adnan2016timeSeriesImproveUserExperience}

% in this work we are doing this to help

% While prior work has established foundational principles of line graph perception~\cite{quadri2021survey}, less is known about how these processes unfold when viewers encounter line charts embedded in real-world contexts, where textual framing and design elements co-occur.

% merge 2.3 and 2.1
% add more citations
% \vspace{-10pt}
\noindent \textbf{Textual Information in Line Charts} Line charts in media rarely appear without accompanying text.
Titles, captions, and annotations collectively guide attention, shape interpretation, and frame the narrative structure of what viewers perceive and remember~\cite{stokes2025analysistextfunctionsinformation, borkin2016beyondMemorability}.
Recent work demonstrates that such textual elements can meaningfully steer attention and shape interpretation, sometimes even overriding the visual data itself~\cite{stokes2022striking, kong2019recallInfoTitleVisualizationMisalignment}.
% 
For example, captions that explicitly reference chart features, such as peaks, valleys, or trends, improve comprehension and support accurate recall of salient patterns, particularly for single-class line charts~\cite{kim2021understandingReadersIntegrateChartsCaptions}.
% Titles, as the most prominent textual element, also exert a strong influence.
Viewers often align their understanding with the message of a title even under conditions of misalignment of the title-data, suggesting that titles function as interpretive anchors~\cite{kong2019recallInfoTitleVisualizationMisalignment}
The strategic use of titles in the news media further complicates this dynamic. Emotionally charged or "slanted" phrasing can distort attention, amplify perceived effects, and guide viewers' emotional responses to visualized data~\cite{kong2018slantsTitles}. However, an in-depth study is needed on variation in title framing and its influence on viewers' perception of pattern interpretation. 

% Despite growing evidence that individual textual elements influence interpretation, prior studies typically isolate a single feature under controlled conditions. News charts, by contrast, present titles, captions, and annotations as co-occurring rhetorical elements shaped by communicative goals~\cite{lauer2020influencedByDeceptiveTactics}. How these naturally co-occurring textual factors relate to viewers' pattern identification remains an open question.

% \subsection{Visual Scaffolding and Structural Cues}
% Beyond text, viewers rely on structural reference cues such as axes, tick marks, and gridlines to make sense of magnitude and change. Prior work has examined how axis design supports value estimation and reading, including algorithms and practices for tick and label placement~\cite{talbot2010algorithmPositioningTickLabelsAxes}. Other studies show that rescaling and y-axis truncation can alter perceived magnitude and trend strength, with effects that depend on task and communicative intent~\cite{fisher2021rescaling, correll2020TruncatingYaxisThreat, long2024yaxisTruncation}. Gridlines and visual hierarchy further influence perceptual organization and attention, and recent work suggests gridlines can improve accuracy for vertical comparisons and slope judgments in line charts~\cite{bartram2011grids, knittel2024gridlines}. This research motivates treating tick marks and gridline presence as meaningful factors that may shape pattern labeling.

